Explaining Counterexamples with Giant-Step Assertion Checking

Identifying the cause of a proof failure during deductive verification of programs is hard: it may be due to an incorrectness in the program, an incompleteness in the program annotations, or an incompleteness of the prover. The changes needed to resolve a proof failure depend on its category, but the prover cannot provide any help on the categorisation. When using an SMT solver to discharge a proof obligation, that solver can propose a model from a failed attempt, from which a possible counterexample can be derived. But the counterexample may be invalid, in which case it may add more confusion than help. To check the validity of a counterexample and to categorise the proof failure, we propose the comparison between the run-time assertion-checking (RAC) executions under two different semantics, using the counterexample as an oracle. The first RAC execution follows the normal program semantics, and a violation of a program annotation indicates an incorrectness in the program. The second RAC execution follows a novel "giant-step" semantics that does not execute loops nor function calls but instead retrieves return values and values of modified variables from the oracle. A violation of the program annotations only observed under giant-step execution characterises an incompleteness of the program annotations. We implemented this approach in the Why3 platform for deductive program verification and evaluated it using examples from prior literature.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{A. Paskevich, J. Proen\c{c}a (Eds.): Formal Integrated\\
Development Environment 2021 (F-IDE 2021)\\
EPTCS 338, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.338.10}{10.4204/EPTCS.338.10}}
\pdfoutput=1

